NEVO-GSPT: Population-Based Neural Network Evolution Using Inflate and Deflate Operators

Evolving neural network architectures is a computationally demanding process. Traditional methods often require an extensive search through large architectural spaces and offer limited understanding of how structural modifications influence model behavior. This paper introduces \gls{ngspt}, a novel Neuroevolution algorithm based on two key innovations. First, we adapt geometric semantic operators~(GSOs) from genetic programming to neural network evolution, ensuring that architectural changes produce predictable effects on network semantics within a unimodal error surface. Second, we introduce a novel operator (DGSM) that enables controlled reduction of network size, while maintaining the semantic properties of~GSOs. Unlike traditional approaches, \gls{ngspt}'s efficient evaluation mechanism, which only requires computing the semantics of newly added components, allows for efficient population-based training, resulting in a comprehensive exploration of the search space at a fraction of the computational cost. Experimental results on four regression benchmarks show that \gls{ngspt} consistently evolves compact neural networks that achieve performance comparable to or better than established methods in the literature, such as standard neural networks, SLIM-GSGP, TensorNEAT, and SLM.

==> hparams.tex <==
\newcommand{\slmGen}{100}
\newcommand{\tneatGen}{1000}
\newcommand{\slmPopsize}{100}
\newcommand{\slmMaxnodes}{627}
\newcommand{\slmMaxConns}{626}

==> imports.tex <==

\usepackage{graphicx}%
\usepackage{multirow}%
\usepackage{amsmath,amssymb,amsfonts}%
\usepackage{mathrsfs}%
\usepackage[title]{appendix}%
\usepackage{xcolor}%
\usepackage{textcomp}%
\usepackage{manyfoot}%
\usepackage{booktabs}%
\usepackage{algorithm}%
\usepackage{algorithmicx}%
\usepackage{algpseudocode}%
\usepackage{listings}%
\usepackage{glossaries}
\usepackage{hyperref}
\usepackage{cleveref}
\usepackage{subcaption}
\usepackage{cancel}
\usepackage[inline]{enumitem}

%all our papers stuff
\usepackage[utf8]{inputenc}

\usepackage{color,colortbl,etoolbox}
\usepackage[linewidth=1pt,ticklabelscale=0.75,titleyshift=-1mm]{plotmacros}

\usetikzlibrary{external}

\usepackage{caption}
\captionsetup{font=small,skip=2pt}  

\usepackage[compact]{titlesec}         % you need this package
\titlespacing{\section}{1pt}{1pt}{1pt} % this reduces space between (sub)sections to 0pt, for example


